A Collaborative PIM Computing Optimization Framework for Multi-Tenant DNN

Modern Artificial Intelligence (AI) applications are increasingly utilizing multi-tenant deep neural networks (DNNs), which lead to a significant rise in computing complexity and the need for computing parallelism. ReRAM-based processing-in-memory (PIM) computing, with its high density and low power consumption characteristics, holds promising potential for supporting the deployment of multi-tenant DNNs. However, direct deployment of complex multi-tenant DNNs on exsiting ReRAM-based PIM designs poses challenges. Resource contention among different tenants can result in sever under-utilization of on-chip computing resources. Moreover, area-intensive operators and computation-intensive operators require excessively large on-chip areas and long processing times, leading to high overall latency during parallel computing. To address these challenges, we propose a novel ReRAM-based in-memory computing framework that enables efficient deployment of multi-tenant DNNs on ReRAM-based PIM designs. Our approach tackles the resource contention problems by iteratively partitioning the PIM hardware at tenant level. In addition, we construct a fine-grained reconstructed processing pipeline at the operator level to handle area-intensive operators. Compared to the direct deployments on traditional ReRAM-based PIM designs, our proposed PIM computing framework achieves significant improvements in speed (ranges from 1.75x to 60.43x) and energy(up to 1.89x).

==> _tab/name.tex <==

\begin{table*}[t]
\caption{Summary of experiments results}
\centering
\captionsetup{singlelinecheck = false, justification=justified, font=footnotesize}
\tabcolsep 2pt
\begin{tabular}{llccccc}

\hline
{\color[HTML]{CB0000} }                 & Multi-tenant DNN & \tabincell{c}{origin \\energy(mJ)}  & \tabincell{c}{optimi \\energy(mJ)}
  & \tabincell{c}{overall \\speedup} & \tabincell{c}{tenant \\contri} & \tabincell{c}{operator \\contri} \\ \hline
   & DNN4+VGG11+VGG16   &19.75 &10.44    & 4.48  & 14\%   & 86\%  \\
   & VGG13+VGG16+VGG19  &37.49 &27.07    & 1.79  & 17\%   & 83\%  \\
   & VGG11+VGG13+VGG19  &33.76  &23.02    & 1.85  & 24\%   & 76\%  \\
   & DNN1+DNN2+DNN3     &17.43  &10.70    & 12.6  & 3.33\% & 97\%  \\
   & DNN2+DNN3+DNN4     &11.57  &12.09    & 22.53 & 6\%    & 94\%  \\
   & DNN1+DNN3+VGG16+VGG19 &36.50  &20.58 & 4.8   & 17\%   & 83\%  \\
   & VG11+VGG13+VGG16+VGG19 &46.42  &35.45 & 1.75  & 48\%   & 52\%  \\
\multirow{-8}{*}{\rotatebox{90}{\tabincell{c}{chip1\\(168-12-8-128)}}}     & DNN1+VGG11+VGG13+VGG16    &37.95  &27.09           & 1.96                                    & 36\%                    & 64\%                \\ \hline
   & DNN4+VGG11+VGG16   &19.69  &15.38    & 5.92  & 7\%    & 93\%  \\
   & VGG13+VGG16+VGG19  &37.42  &38.83    & 1.98  & -29\%  & 129\% \\
   & VGG11+VGG13+VGG19  &33.69  &32.33    & 2.17  & -5\%   & 105\% \\
   & DNN1+DNN2+DNN3     &17.40  &13.19    & 16.15 & 2.00\% & 98\%  \\
   & DNN2+DNN3+DNN4     &11.56  &12.09    & 30.85 & 0\%    & 100\% \\
   & DNN1+DNN3+VGG16+VGG19 &36.50  &31.50 & 7.2   & 12\%   & 88\%  \\
   & VG11+VGG13+VGG16+VGG19 &46.42  &46.40   & 2.01  & 9\%    & 91\%  \\
\multirow{-8}{*}{\rotatebox{90}{\tabincell{c}{chip2\\(256-12-12-128)}}}    & DNN1+VGG11+VGG13+VGG16    &37.95  &35.44           & 2.32                                & 11\%                & 89\%            \\ \hline
   & DNN4+VGG11+VGG16   &19.65  &20.45    & 8.06  & 0\%    & 100\% \\
   & VGG13+VGG16+VGG19  &37.35  &38.84    & 3.21  & 0\%    & 100\% \\
   & VGG11+VGG13+VGG19  &33.62  &34.94    & 3.67  & 8\%    & 92\%  \\
   & DNN1+DNN2+DNN3     &17.38  &18.16    & 31.12 & 0.00\% & 100\% \\
   & DNN2+DNN3+DNN4     &11.54  &12.11    & 60.43 & 0\%    & 100\% \\
   & DNN1+DNN3+VGG16+VGG19 &36.50  &36.49  & 9.74  & 3\%    & 97\%  \\
   & VG11+VGG13+VGG16+VGG19 &46.42  &46.42 & 2.81  & -8\%   & 108\% \\
\multirow{-8}{*}{\rotatebox{90}{\tabincell{c}{chip3\\(512-12-12-128)}}}    & DNN1+VGG11+VGG13+VGG16    &37.95  &37.93           & 3.51                                & -0.23\%             & 100.23\%        \\ \hline
\end{tabular}
\label{tab:results}
\vspace{-6mm}
\end{table*}

==> _tab/pseudocode.tex <==
%【整体算法伪码】

\renewcommand{\algorithmicrequire}{\textbf{Input:}}  % Use Input in the format of Algorithm
\renewcommand{\algorithmicensure}{\textbf{Output:}} % Use Output in the format of Algorithm

\begin{algorithm}[htbp]
  \caption{A tenant-operator joint optimization algorithm for multi-tenant DNNs} % 名称
  \label{alg::jointoptimization}
  \begin{algorithmic}[1]
    \Require
      $s_i$: network structure for tenant $i$;
      $s_c$: architecture of accelerator;
      $l$: acceptable delay between tenants;
    \Ensure
      deployment $d$
    \State initial $a_1$ = $a_2$ = $a_3$ = 1/3 computational area;
    
    
    \Function{allocateArea}{$s_1, s_2, s_3, s_c$}
    \While {$delay > l$}
        \State iterAllocation($a_1$,$a_2$,$a_3$)
        \State $t_i$ = processingTime($s_i$,$a_i$)
        \State delay = max($t_1$,$t_2$,$t_3$) - min($t_1$,$t_2$,$t_3$)
    \EndWhile
    \EndFunction
    \Function{processingTime}{$s_i$, $a_i$}
        \State gridSearch($\alpha$ , $\beta$)
        \State re-Op = duplicateandSplit($s_i$,$\alpha$,$\beta$)
        \State $time_{\alpha,\beta}$ = naiveDeploy(re-OP,$a_i$)
        \State save $time_{\alpha,\beta}$
        \State return min(time)
    \EndFunction
  \end{algorithmic}
\end{algorithm}
\vspace{-10pt}
